Dynamic Beveridge Curve Accounting

We develop a dynamic decomposition of the empirical Beveridge curve, i.e., the level of vacancies conditional on unemployment. Using a standard model, we show that three factors can shift the Beveridge curve: reduced-form matching efficiency, changes in the job separation rate, and out-of-steady-state dynamics. We find that the shift in the Beveridge curve during and after the Great Recession was due to all three factors, and each factor taken separately had a large effect. Comparing the pre-2010 period to the post-2010 period, a fall in matching efficiency and out-of-steady-state dynamics both pushed the curve upward, while the changes in the separation rate pushed the curve downward. The net effect was the observed upward shift in vacancies given unemployment. In previous recessions changes in matching efficiency were relatively unimportant, while dynamics and the separation rate had more impact. Thus, the unusual feature of the Great Recession was the deterioration in matching efficiency, while separations and dynamics have played significant, partially offsetting roles in most downturns. The importance of these latter two margins contrasts with much of the literature, which abstracts from one or both of them. We show that these factors affect the slope of the empirical Beveridge curve, an important quantity in recent welfare analyses estimating the natural rate of unemployment.

==> match_fun_table_3s.tex <==
\sisetup{                                                                             
  input-symbols=(),                                                                   
  table-format=-1.5,                                                                  
  table-space-text-post=***,                                                          
  table-align-text-post=false,                                                        
  group-digits=false                                                                  
}                                                                                     
\begin{tabular}{SSSS}                                                                 
 {Sample} & {Specification}  & {$\ln \overline{\sigma}$} & {$\alpha$} \\ \hline \hline
{Full} & {U} & -1.11*** & 0.36*** \\                                                  
 &           & (0.01) & (0.01) \\                                                     
{Pre-2008} & {U} & -1.12*** & 0.29*** \\                                              
 &           & (0.01) & (0.01) \\                                                     
{Post-2008} & {U} & -1.33*** & 0.26*** \\                                             
 &           & (0.01) & (0.01) \\                                                     
{Full} & {U+N} & -0.63*** & 0.43*** \\                                                
 &           & (0.02) & (0.01) \\                                                     
{Pre-2008} & {U+N} & -0.75*** & 0.34*** \\                                            
 &           & (0.02) & (0.01) \\                                                     
{Post-2008} & {U+N} & -0.92*** & 0.33*** \\                                           
 &           & (0.03) & (0.01)                                                        
\end{tabular}                                                                         


==> taylor_decomp_table_gr.tex <==
                                                     
\begin{tabular}{l|c}                                 
Margin &  Contribution (Log Points) \\ \hline \hline 
OOSS Dynamics &  54.75 \\                            
Separations &  -79.28 \\                             
Matching Efficiency &  49.01 \\ \hline               
Total Shift &  24.48                                 
\end{tabular}                                        

